Two simulations about DPLL(T)

In this paper we relate different formulations of the DPLL(T) procedure. The first formulation is based on a system of rewrite rules, which we denote DPLL(T). The second formulation is an inference system of, which we denote LKDPLL(T). The third formulation is the application of a standard proof-search mechanism in a sequent calculus LKp(T) introduced here. We formalise an encoding from DPLL(T) to LKDPLL(T) that was, to our knowledge, never explicitly given and, in the case where DPLL(T) is extended with backjumping and Lemma learning, never even implicitly given. We also formalise an encoding from LKDPLL(T) to LKp(T), building on Ivan Gazeau's previous work: we extend his work in that we handle the "-modulo-Theory" aspect of SAT-modulo-theory, by extending the sequent calculus to allow calls to a theory solver (seen as a blackbox). We also extend his work in that we handle advanced features of DPLL such as backjumping and Lemma learning, etc. Finally, we re fine the approach by starting to formalise quantitative aspects of the simulations: the complexity is preserved (number of steps to build complete proofs). Other aspects remain to be formalised (non-determinism of the search / width of search space).

==> Macros/Macros_10Fomega.tex <==
%Reduction rules
\newcommand\limp{\Rightarrow}

\newcommand{\andorl}{{\land\lor_l}}
\newcommand{\andorr}{{\land\lor_r}}
\newcommand{\andor}{\andorl,\andorr}
\newcommand{\ea}{\forall\exists}
\newcommand{\redF}{\FomegaC}

%Derivability

\newcommand\DerFomT[3]{\Deri[\FomegaC]{#1}{#2}{#3}}
\newcommand\DerFomTs[4]{\Deris[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\Derwf[2]{\textsf{wf}_{#1}(#2)}
\newcommand\DerFomt[4]{\Derif[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\DerFomp[3]{\Derif[\FomegaC]{#1}{#2}{#3}\diamond}

%Syntax
%Kinds

\newcommand\Arr[2]{{#1}\rightarrow {#2}}

%Types
\newcommand{\varT}{\textsf{Var}^T}
\newcommand{\fall}[3][{}]{\forall{#2}^{#1}.{#3}}
\newcommand{\xists}[3][{}]{\exists{#2}^{#1}.{#3}}
\newcommand{\et}[2]{{#1}\wedge {#2}}
\newcommand{\ou}[2]{{#1}\vee {#2}}
%\newcommand{\impl}[2]{{#1}\arr {#2}}
\newcommand{\nega}[1]{\overline{#1}}
\newcommand{\non}[1]{{#1}^{\perp}}
\newcommand{\lamb}[3]{\lambda{#2}^{#1}.{#3}}
\newcommand{\dual}[1]{{#1}^{\bot}}
\newcommand{\bidual}[1]{{#1}^{\bot\bot}}
\newcommand{\tridual}[1]{{#1}^{\bot\bot\bot}}

\newcommand\xistscod[3][{}]{\exists^{\textsf{cod}}{#2}^{#1}.{#3}}
\newcommand{\etcod}[2]{{#1}\wedge^{\textsf{cod}} {#2}}
\newcommand{\oucod}[2]{{#1}\vee^{\textsf{cod}} {#2}}


%Terms
\newcommand\proji[2]{#1}
\newcommand\projii[2]{#2}

\newcommand{\var}{\textsf{Var}}

%\newcommand{\lamc}[4][{}{}]{{#2}^{\i #1}{#3}^{\ii #1}.{#4}}
%\newcommand\stac[2]{{#1}\cdot{{#2}}}
\newcommand{\inj}[4][{}{}]{\lambda #2^{\proji #1}#3^{\projii #1}.{#4}}
\newcommand\paire[2]{\langle{#1},{#2}\rangle}
%\newcommand{\switch}[1]{\bullet #1}

\newcommand{\Lamb}[3]{\Lambda{#2}^{#1}.{#3}}
\newcommand{\appl}[2]{\langle #1,#2\rangle}

\newcommand{\cutc}[2]{\{#1\sep#2\}}

\newcommand{\m}[3][{}]{\mu #2^{#1}\!.{#3}}
%\newcommand{\mt}[3][{}]{\tilde\mu {#2}^{#1}.{#3}}



%Semantics:

\newcommand{\semK}[1]{[\![#1]\!]}
\newcommand{\swapK}[2]{\textsf{swap}_{#1}{#2}}

\newcommand{\sem}[2]{[\![#2]\!]_{#1}}
\newcommand{\semt}[1]{[\![#1]\!]}

\newcommand{\orth}[2]{{#1\mathrel{{\perp}}#2}}

\newcommand{\effac}[1]{\|{#1}\|}
\newcommand{\twt}{\mathcal{T}}

\newcommand{\mU}{\mathcal U}
\newcommand{\mV}{\mathcal V}

\newcommand{\fp}[2]{\Phi_{#1}{#2}}
\newcommand\LamC[1]{\Lambda\_.{#1}}
\newcommand\applC[1]{\appl{\_}{#1}}

%======================
%Relationship with other formalisms

\newcommand\FFc[2][]{\delambda[#1]{(#2)}}
\newcommand\FFct[2]{\delambda({#2},{#1})}
\newcommand\FFctv[1]{\delambda{(#1)}}
\newcommand\FcFp[1]{{#1}^+}
\newcommand\FcFm[1]{{#1}^-}
\newcommand\FcFt[1]{#1^\dagger}
\newcommand\cstc{{\textsf{C}}}

\newcommand\FFctvname{\delambda[\textsf{V}]}

%Derivability in Fomega normal

\newcommand\DerFomiT[3]{\Deri[\Fomega]{#1}{#2}{#3}}
\newcommand\DerFomitwf[2]{\textsf{wf}^{#1}_{\Fomega}(#2)}
\newcommand\DerFomit[4]{\Derif[\Fomega]{#1}{#2}{#3}{#4}}

\newcommand\SNC{\SN{\B'\x'}_{\textsf{TC}}}
\newcommand\SNl{\SN{\B'\x'}_{\textsf{TL}}}


==> Macros/Macros_3CBV.tex <==
\newcommand\CPS{\textsf{CPS}}

%Moggi's lC
\newcommand\letinC[3]{\textsf{let }#2=#1\textsf{ in }{#3}}

\newcommand\bv{\beta_{\textsf V}}
\newcommand\ev{\eta_{\textsf V}}
\newcommand\evp{\eta'_{\textsf V}}


\newcommand\bl{{\textsf {B}}}
\newcommand\letC{{\textsf {let}}_{\textsf V}}
\newcommand\appleti{{\textsf {let}}_1}
\newcommand\appletii{{\textsf {let}}_2}
\newcommand\etalet{\eta_{\textsf {let}}}
\newcommand\letnesting{{\textsf {assoc}}}

%\newcommand\lCx{\lambda_{{\textsf C}\textsf{x}}}
\newcommand\lCb{\lambda_{{\textsf C}\beta}}
\newcommand\lCbe{\lambda_{{\textsf C}\beta\eta}}

%CPS-translations
\renewcommand\Re[1]{\mathcal{R}(#1)}
\newcommand\ReV[1]{\mathcal{R}_{\textsf V}(#1)}
\newcommand\Fi[1]{\mathcal{F}(#1)}
\newcommand\FiV[1]{\mathcal{F}_{\textsf V}(#1)}

\newcommand\Fis[2]{{#1}\colon_{\!\!\mathcal{F}}{#2}}
\newcommand\FisV[1]{{#1}^{\mathcal F}}
\newcommand\Rey[2]{{#1}\colon_{\!\!\mathcal{R}}{#2}}
\newcommand\ReyV[1]{{#1}^{\mathcal R}}

\newcommand\Fisback[1]{{#1}^{{\mathcal F}{\textsf {back}}}}
\newcommand\Fisbackname{{\mathcal F}{\textsf {back}}}


%Calculs CPS
\newcommand\lav{$\lambda_{\textsf {EvalArg}}$}
\newcommand\lContR{$\lambda^{\mathcal R}_{\CPS}$}
\newcommand\lContF{$\lambda^{\mathcal F}_{\CPS}$}
\newcommand\lContp{$\lambda_{\CPS}^+$}

\newcommand\lContRb{\lambda^{\mathcal R}_{\CPS\beta}}
\newcommand\lContRbe{\lambda^{\mathcal R}_{\CPS\beta\eta}}
\newcommand\lContFb{\lambda^{\mathcal F}_{\CPS\beta}}
\newcommand\lContFbe{\lambda^{\mathcal F}_{\CPS\beta\eta}}

\newcommand\lif[1]{\Uparrow{#1}}
\newcommand\lifname{\Uparrow}

%For later

\newcommand\lContfb{\lambda^{f}_{\CPS\beta}}
\newcommand\lContfbe{\lambda^{f}_{\CPS\beta\eta}}

\newcommand\nnot[1]{{#1}^{\bullet}}

\newcommand\liFf[1]{\uparrow{#1}}
\newcommand\liFfname{\uparrow}

\newcommand\cps[2]{{#1}\colon{#2}}
\newcommand\cpsV[1]{{#1}^{\dag}}

\newcommand\spc[1]{{#1}^{{\textsf {back}}}}
\newcommand\spcname{{(\_)}^{{\textsf {back}}}}

\newcommand\lContf{$\lambda^{f}_{\CPS}$}

\newcommand\lCont{\lambda_{\CPS}}

\newcommand\lConti{\lambda_{\textsf{cont}1}}
\newcommand\lContii{\lambda_{\textsf{cont2}}}

%To and from Moggi's C

\newcommand\Tii[1]{{#1}^{\sharp}}
\newcommand\Tiii[1]{{#1}^\natural}
\newcommand\Ti[1]{{#1}^\flat}

%\newcommand\Tiname{{(\_)}^\flat}
%\newcommand\Tiiname{{(\_)}^\sharp}
%\newcommand\Tiiiname{{(\_)}^\natural}


==> Macros/Macros_4LambdaI.tex <==
%lambda I

\renewcommand\corner[1]{\v{#1}}
\newcommand\wonalc{$\l^?$}
\newcommand\subanot[2]{#1\lhd{#2}}

\renewcommand\P[3]{\Pi {#1}^{#2}.{#3}}
\newcommand\lami[3]{\lambda {#1}^{#2}.{#3}}

\newcommand\dummy{\wp}
\renewcommand\i[1]{\textsf{i}({#1})}
\newcommand\iname{\textsf{i}}

\newcommand\typ{t}
\newcommand\betat{{\beta^{\typ}}}

\newcommand\pervar{\textsf{perp-var}}
\newcommand\perl{\textsf{perp}\lambda}
\newcommand\perlaa{\textsf{perp}\lambda^{\typ}_1}
\newcommand\perlab{\textsf{perp}\lambda^{\typ}_2}
\newcommand\perba{\textsf{perp}\beta_1}
\newcommand\perbb{\textsf{perp}\beta_2}
\newcommand\perbaa{\textsf{perp}\betat_1}
\newcommand\perbba{\textsf{perp}\betat_2}
\newcommand\perbca{\textsf{perp}\betat_3}
\newcommand\perpia{\textsf{perp}\Pi_1}
\newcommand\perpib{\textsf{perp}\Pi_2}

\newcommand\per{\rightsquigarrow}

\newcommand\RI[2]{{#1}\;\mathcal H\;{#2}}

\newcommand\GI[2]{{#1}\;\mathcal{G}\;{#2}}
\newcommand\Gax{\mathcal{G}\textsf{ax}}
\newcommand\Gvar{\mathcal{G}\textsf{var}}
\newcommand\Gl{\mathcal{G}\lambda}
\newcommand\Gla{\mathcal{G}\lambda^{\typ}}
\newcommand\Gba{\mathcal{G}\beta_1}
\newcommand\Gbb{\mathcal{G}\beta_2}
\newcommand\Gbaa{\mathcal{G}\betat_1}
\newcommand\Gbba{\mathcal{G}\betat_2}
\newcommand\Gweak{\mathcal{G}\textsf{weak}}
\newcommand\Gweaka{\mathcal{G}\textsf{weak1}}
\newcommand\Gweakb{\mathcal{G}\textsf{weak2}}
\newcommand\Gc{\mathcal{G}\textsf{c}}
\newcommand\Gpi{\mathcal{G}\textsf{$\Pi$}}

==> Macros/Macros_4SafeMin.tex <==
%PSN & Encodings to and from lambda=======================

\newcommand{\PSN}{{\textsf{PSN}}}


\renewcommand\H[1]{\textsf{H}({#1})}
\newcommand\Hname{\textsf{H}}
\newcommand\xtol[1]{\H{#1}}
\newcommand\xtolname{\Hname}

\newcommand\delambda[1][]{{\mathcal A}_{#1}}
\newcommand\alambda{{\mathcal B}}
\newcommand\dd[1]{\delambda(\alambda({#1}))}

\newcommand\kC[1]{{\delambda}_{\textsf{w}}{({#1})}}
\newcommand\kCCC[1]{{\delambda}{(#1)}}
\newcommand\kCC[2][]{{\delambda}_{#1}{(#2)}}
\newcommand\kCCname{{\delambda}}

\renewcommand\k[1]{\alambda{(#1)}}
\newcommand\kl[2]{\alambda^{#1}{(#2)}}
\newcommand\kname{{\mathcal B}}


%RPO encoding

\newcommand\polyx[1]{\overline{#1}}
\newcommand\polyxname{\overline {(\;)}}
\newcommand\polyxg[1]{\polyx{#1}}
\newcommand\polyxgname{\polyxname}


\newcommand\nb[1]{\sharp #1}

\newcommand\fo[1]{\polyx {#1}}
\newcommand\foe[1]{\polyx {#1}}
\newcommand\foename{\polyxname}

\newcommand\fot[1]{\polyx {#1}}
\newcommand\fotname{\polyxname}


\ignore{
\newcommand\polyx[1]{\mathcal P(#1)}
\newcommand\polyxname{\mathcal P}
}


%Safeness and minimality

\newcommand\safe[1]{\textsf{safe} {#1}}
\newcommand\minim[2]{\textsf{min}_{#1} #2}
\renewcommand\min[1]{\minim{}{#1}}

\newcommand{\unsafe}[1]{{\stackrel{\textsf{unsafe}}\longrightarrow}_{#1}\;}
\newcommand{\unsafen}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}
\newcommand{\unsafeplus}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{+}}_{#1}\;}
\newcommand{\undafesn}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}


%Lambda x
\newcommand\lamp[3]{\lambda {#1}.{#3}}
\newcommand\cuti[4]{\langle{#2}/{#3}\rangle{#4}}

\newcommand\x{\textsf{x}}



==> Macros/Macros_5Llxr.tex <==
\newcommand\strict{basic}
\newcommand\expsub{substitution constructor}

%Rewriting specific===========================

\newcommand{\Sim}[1]{\sim_{#1}\;}
\newcommand{\Rewmod}[2]{\rightarrow_{#1/#2}\;}
\newcommand{\Rewmodn}[2]{\rightarrow^{*}_{#1/#2}\;}

\newcommand{\LRewplus}[1]{\; \mbox{}_{#1}^{+}{\longleftarrow}\;}
\newcommand{\LRew}[1]{\; \mbox{}_{#1}{\longleftarrow}}
\newcommand{\LRewn}[1]{\; {\mbox{}_{#1\,}}^{*}{\longleftarrow}}
\newcommand{\RLRewn}[1]{{\longleftrightarrow}^{*}_{#1}}
\newcommand{\RLRew}[1]{{\longleftrightarrow}_{#1}}


\newcommand{\ssubst}[3]{\subst{#1}{#3}{#2}}
%\newcommand{\isubst}[2]{\{ #1 \backslash #2 \} }



%Terms===========================

\renewcommand\t{\textsf{r}}
\newcommand\xt{\textsf{xr}}
\newcommand{\weak}[2]{\mathcal{W}_{#1}(#2)}
\newcommand{\app}[4]{#1\; #3}

\newcommand{\clos}[2]{#2 {#1}}
\newcommand{\trip}[3]{\cuti{}{#2} {#1}}

%\newcommand{\clos}[2]{#1\langle #2\rangle}
%\newcommand{\trip}[3]{#1 =_{#3} #2}
%\newcommand{\iclos}[2]{#1[#2]}
\newcommand{\con}[4]{\mathcal{C}_{#1}^{#2\,|\,#3}(#4)}

\newcommand{\weakapp}[5]{\weak {#1}{\app {#2}{} {#4}{}}}

\newcommand{\wf}{\mbox{ \textsf{linear}}}

%Equations======================
\newcommand{\ac}{\textsf{A}_{\textsf{c}}}
\newcommand{\ccu}{\textsf{C}_{\textsf{c}}}
\newcommand{\ccd}{\textsf{P}_{\textsf{c}}}
\newcommand{\cw}{\textsf{P}_{\textsf{w}}}
\newcommand{\com}{\textsf{P}_{\textsf{s}}}
\newcommand{\cs}{\textsf{P}_\textsf{cs}}


%Rules============================

\newcommand\Abs{\textsf{Abs}}
\newcommand\Appi{\textsf{App1}}
\newcommand\Appii{\textsf{App2}}
\newcommand\Var{\textsf{Var}} 
\newcommand\Weaki{\textsf{Weak1}}
\newcommand\Weakii{\textsf{Weak2}}
\newcommand\Cont{\textsf{Cont}}
\newcommand\Comp{\textsf{Comp}}
\newcommand\WAbs{\textsf{WAbs}}
\newcommand\WAppi{\textsf{WApp1}}
\newcommand\WAppii{\textsf{WApp2}}
\newcommand\WSubs{\textsf{WSubs}} 
\newcommand\Merge{\textsf{Merge}}
\newcommand\Cross{\textsf{Cross}}
\newcommand\CAbs{\textsf{CAbs}}
\newcommand\CAppi{\textsf{CApp1}} 
\newcommand\CAppii{\textsf{CApp2}} 
\newcommand\CSubs{\textsf{CSubs}}

%Translation=================

\newcommand{\ord}[1]{{#1}}

%sn-x=========================
\newcommand\multip[2]{\mathcal M_{#1}({#2})}
\newcommand\Tcomplex[1]{\mathcal {T}\!\textsf{x} ({#1})}
\newcommand\pol[1]{\mathcal P({#1})}
\newcommand\polname{\mathcal P}

==> Macros/Macros_6G3.tex <==
%Strategies
\newcommand\princ{{\textsf{princ}}}
\newcommand\gauche{\textsf{left}}
\newcommand\droite{\textsf{right}}

\newcommand\simpl{{\textsf{s}}}
\newcommand\SI{{\textsf{SI}}}
\newcommand\KK{{\textsf{KK}}}
\newcommand\JC{{\textsf{JC}}}

\newcommand\CBV{\textsf{CBV}}
\newcommand\CBN{\textsf{CBN}}
\newcommand\CBVs{\textsf{CBV}_{\textsf{simple}}}
\newcommand\CBNs{\textsf{CBN}_{\textsf{simple}}}
\newcommand\CB{\textsf{CB}}
\newcommand\equCBV{\equiv_{\CBV}}
\newcommand\equCBN{\equiv_{\CBN}}

\newcommand\clas{\equiv}
\newcommand\mogo{\textsf{sc}}
\newcommand\quot{\textsf{nd}}

\newcommand\purq{\textsf{pur-q}}
\newcommand\purt{\textsf{pur-t}}
\newcommand\purGp{\textsf{pur}\Giiii'}
\newcommand\purGiv{\textsf{pur}\Giv}


%lambdabar

\newcommand\SVar{{\mathcal X}}
\newcommand\STerms{{\mathcal T}}
\newcommand\SLists{{\mathcal L}}

\newcommand\TSVar{{\mathcal Y}}
\newcommand\PSVar{{\mathcal X}}
\newcommand\TS{{\mathcal P}}
\newcommand\PSTerms{{\mathcal T}}
\newcommand\PSLists{{\mathcal L}}


\newcommand\cont[2]{{#1}\;{#2}}

\newcommand\el{[]}
\newcommand\conc[2]{{#1}@{#2}}
\newcommand\st[2]{{#1}\cdot{#2}}

%Typing
\newcommand\contr[1]{\textsf{select}_{#1}}

\newcommand\Air{\rightarrow\textsf{r}}
\newcommand\Ail{\rightarrow\textsf{l}}


%Term reduction rules
\newcommand\B{\textsf{B}}
\newcommand\Ai{\textsf{A1}}
\newcommand\Aii{\textsf{A2}}
\newcommand\Aiii{\textsf{A3}}
\newcommand\Bi{\textsf{B1}}
\newcommand\Bii{\textsf{B2}}
\newcommand\Biii{\textsf{B3}}
\newcommand\Ci{\textsf{C1}}
\newcommand\Cii{\textsf{C2}}
\newcommand\Ciii{\textsf{C3}}
\newcommand\Civ{\textsf{C4}}
\newcommand\Cv{\textsf{C5}}
\newcommand\Cvi{\textsf{C6}}
\newcommand\Cvii{\textsf{C7}}
\newcommand\Cviii{\textsf{C8}}
\newcommand\Di{\textsf{D1}}
\newcommand\Dii{\textsf{D2}}
\newcommand\Diii{\textsf{D3}}
\newcommand\Div{\textsf{D4}}
%\newcommand\Ei{\textsf{E}}
%\newcommand\Fi{\textsf{F}}

\newcommand\As{\textsf{As}}
\newcommand\Bs{\textsf{Bs}}
\newcommand\Cs{\textsf{Cs}}
\newcommand\CGs{\textsf{Cs}_{\textsf G}}
\newcommand\Ds{\textsf{Ds}}
\newcommand\Es{\textsf{E}}

==> Macros/Macros_7G4.tex <==
\def\ijcar{}
\def\journal{\ignore}
%=================================================

\newcommand{\Lveerto}{\mbox{$L\!\vee\!\rto$}}

\newcommand{\AB}{A\rto B}
\newcommand{\BA}{B\rto A}

\newcommand{\BC}{B\rto C}

\newcommand{\ABC}{(\AB) \rto C}
\newcommand{\CD}{C\rto D}
\newcommand{\DB}{D\rto B}
%\newcommand{\CB}{C\rto B}
\newcommand{\FG}{F\rto G}
\newcommand{\GH}{G\rto H}
\newcommand{\CDB}{(\CD)\rto B}
\newcommand{\FGH}{(\FG)\rto H}

\newcommand{\dec}[2]{\mbox{${#1}\!\colon\!{#2}$}}
\newcommand{\vA}{\mbox{$\dec{v}{A}$}}
\newcommand{\vB}{\mbox{$\dec{v}{B}$}}
\newcommand{\uC}{\mbox{$\dec{u}{C}$}}
\newcommand{\vC}{\mbox{$\dec{v}{C}$}}
\newcommand{\wA}{\mbox{$\dec{w}{A}$}}
\newcommand{\wB}{\mbox{$\dec{w}{B}$}}
\newcommand{\wC}{\mbox{$\dec{w}{C}$}}
\newcommand{\wD}{\mbox{$\dec{w}{D}$}}
\newcommand{\wE}{\mbox{$\dec{w}{E}$}}
\newcommand{\xA}{\mbox{$\dec{x}{A}$}}
\newcommand{\xB}{\mbox{$\dec{x}{B}$}}
\newcommand{\xC}{\mbox{$\dec{x}{C}$}}
\newcommand{\yA}{\mbox{$\dec{y}{A}$}}
\newcommand{\yB}{\mbox{$\dec{y}{B}$}}
\newcommand{\yC}{\mbox{$\dec{y}{C}$}}
\newcommand{\yD}{\mbox{$\dec{y}{D}$}}
\newcommand{\yE}{\mbox{$\dec{y}{E}$}}
\newcommand{\zA}{\mbox{$\dec{z}{A}$}}
\newcommand{\zB}{\mbox{$\dec{z}{B}$}}
\newcommand{\zC}{\mbox{$\dec{z}{C}$}}
\newcommand{\zD}{\mbox{$\dec{z}{D}$}}
\newcommand{\zE}{\mbox{$\dec{z}{E}$}}
\newcommand{\MA}{\mbox{$\dec{M}{A}$}}
\newcommand{\MB}{\mbox{$\dec{M}{B}$}}
\newcommand{\MD}{\mbox{$\dec{M}{D}$}}
\newcommand{\ME}{\mbox{$\dec{M}{E}$}}
\newcommand{\NA}{\mbox{$\dec{N}{A}$}}
\newcommand{\NB}{\mbox{$\dec{N}{B}$}}
\newcommand{\ND}{\mbox{$\dec{N}{D}$}}
\newcommand{\NE}{\mbox{$\dec{N}{E}$}}


                    
\ignore{
\newcommand{\esapp}[4]{\langle\!\langle #1/#2, #3,#4  \rangle    \!   \rangle}
\newcommand{\esappt}[3]{\langle\!\langle #1/#2, #3  \rangle    \!   \rangle}
\newcommand{\tesapp}[1]{\langle\!\langle #1 \rangle  \! \rangle}
\newcommand{\nomtesapp}{\langle\!\langle ~ \rangle \!\rangle}
\newcommand{\tsapp}[1]{\{\!\{ #1 \}  \! \}}
\newcommand{\nomtsapp}{\{ \! \{ ~ \} \! \}}
\newcommand{\sapp}[3]{\{\!\{#1/#2,#3 \}\! \}}
\newcommand{\ce}[2]{[\![#1/#2]\!]}
\newcommand{\nomcut}{cut}
\newcommand{\tcut}[2]{cut(#1,#2)}
\newcommand{\la}[4]{{\tt app}(#1,#2,#3.#4)}
\newcommand{\rew}{\rightarrow}
%\newcommand{\tra}[1]{{\cal T}(#1)}
\newcommand{\tra}[1]{\overline{#1}}
%\newcommand{\tce}[4]{[\![#4]\!]_{#1,#2,#3}}
\newcommand{\tce}[2]{[\![#2]\!]_{#1}}
\newcommand{\nomtce}{[\![~]\!]_{A}}
\newcommand{\tes}[2]{[#2]_{#1}}
\newcommand{\nomtes}{[~]_{A}}



\newcommand{\spred}{\triangleright}
\newcommand{\pair}[2]{\langle #1,#2\rangle}
\newcommand{\triple}[3]{\langle #1,#2,#3\rangle}
\newcommand{\app}[2]{app(#1,#2)}
\newcommand{\tapp}[3]{app(#2,#3)_{#1}}
\newcommand{\nomtapp}{app_{A}}
\newcommand{\msep}{\hspace{.5cm}}
}

\newcommand{\lam}[2]{\lambda {#1}.{#2}}
\newcommand{\leftz}[4]{#1[#2,#3.#4]}
\newcommand{\leftr}[6]{#1[#2.#3.#4,#5.#6]}
\newcommand{\inv}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninv}{{\tt inv}}
\newcommand{\inva}[2]{{\tt inva}(#1,#2)}
\newcommand{\invz}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninvz}{{\tt inv}}
\newcommand{\invr}[3]{{\tt inv}(#1,#2.#3)}

\newcommand{\type}[1]{\widehat{#1}}
%\newcommand{\of}[2]{#1 \; {\tt of }\; #2}
\newcommand{\of}[2]{{\tt of}(#1,#2)}
\newcommand{\nof}{{\tt of}}
\newcommand{\Of}{O\! f}
\newcommand{\Inv}{Inv}
\newcommand{\genax}[2]{{\tt Ax}(#1,#2)}
\newcommand{\decomp}[4]{{\tt dec}(#1,#2,#3.#4)}
\newcommand{\ndecomp}{{\tt dec}}
%\renewcommand{\ar}[3]{(#1 \rto #2) \rto #3}

\newcommand{\Cut}[3]{\letin {#1}{#2}{#3}}
\newcommand{\ncut}{{\tt cut}}

%========================
%Rewrite rules

\newcommand\decri{\textsf{d}1}
\newcommand\decrii{\textsf{d}2}
\newcommand\decriii{\textsf{d}3}
\newcommand\decriv{\textsf{d}4}
\newcommand\decrv{\textsf{d}5}
\newcommand\decrvi{\textsf{d}6}
\newcommand\decrvii{\textsf{d}7}
\newcommand\decrviii{\textsf{d}8}

\newcommand\cutri{\textsf{c}1}
\newcommand\cutrii{\textsf{c}2}
\newcommand\cutriii{\textsf{c}3}
\newcommand\cutriv{\textsf{c}4}
\newcommand\cutrv{\textsf{c}5}
\newcommand\cutrvi{\textsf{c}6}
\newcommand\cutrvii{\textsf{c}7}
\newcommand\cutrviii{\textsf{c}8}
\newcommand\cutrix{\textsf{c}9}

\ignore{
\newcommand\cutrx{\textsf{c}{10}}
\newcommand\cutrxi{\textsf{c}{11}}
\newcommand\cutrxii{\textsf{c}{12}}
\newcommand\cutrxiii{\textsf{c}{13}}
\newcommand\cutrxiv{\textsf{c}{14}}
\newcommand\cutrxv{\textsf{c}{15}}
\newcommand\cutrxvi{\textsf{c}{16}}
}

\ignore{
\newcommand\cutri{a}
\newcommand\cutrii{b}
\newcommand\cutriii{c}
\newcommand\cutriv{d}
\newcommand\cutrv{e}
\newcommand\cutrvi{f}
\newcommand\cutrvii{g}
\newcommand\cutrviii{\pi}
\newcommand\cutrix{\phi}
}
\newcommand\cutrx{\textsf{A}}
\newcommand\cutrxi{\textsf{B}}
\newcommand\cutrxii{\textsf{C}}
\newcommand\cutrxiii{\textsf{D}}
\newcommand\cutrxiv{\textsf{E}}
\newcommand\cutrxv{\textsf{F}}
\newcommand\cutrxvi{\textsf{G}}


\newcommand\invi{\textsf{i}1}
\newcommand\invii{\textsf{i}2}
\newcommand\inviii{\textsf{i}3}
\newcommand\inviv{\textsf{i}4}
\newcommand\invv{\textsf{i}5}
\newcommand\invvi{\textsf{i}6}
\newcommand\invvii{\textsf{i}7}
\newcommand\invviii{\textsf{i}8}

\newcommand\ofi{\textsf{o}1}
\newcommand\ofii{\textsf{o}2}
\newcommand\ofiii{\textsf{o}3}
\newcommand\ofiv{\textsf{o}4}

\newcommand{\lz}{L0 \rto}
\newcommand{\lrr}{L \rto\rto}

\ignore{
\newcommand{\lzn}{Lb}
\newcommand{\lrrn}{Li}
}
\newcommand{\lzn}{\textsf{I}}
\newcommand{\lrrn}{\textsf{K}}
\newcommand{\foA}{\textsf{I}}
%\newcommand{\fo}{\star}
\newcommand{\foI}{\textsf{J}}
\newcommand{\foO}{\textsf{J}}
\newcommand{\fodec}[1]{\textsf{D}^{#1}}
\newcommand{\foCut}[1]{\textsf{C}^{#1}}


\newcommand{\oid}{{\sf{ivdc}}}
\newcommand{\oidgs}{{\sf{ivdcgs}}}
\newcommand{\gs}{{\sf{gs}}}
\newcommand{\cegs}{{\sf{cegs}}}
\newcommand{\rs}{{\sf{rs}}}
\newcommand{\cers}{{\sf{cers}}}
\newcommand{\ars}{{\sf{ars}}}
\newcommand{\cears}{{\sf{cears}}}
\newcommand{\cbn}{{\sf{cbn}}}
\newcommand{\cecbn}{{\sf{cecbn}}}
\newcommand{\cbv}{{\sf{cbv}}}
\newcommand{\cecbv}{{\sf{cecbv}}}

\newcommand{\pr}{Principal}
\newcommand{\np}{Non-Principal}
\newcommand{\na}{Non-Auxiliary}
\newcommand{\au}{Auxiliary}

\def\kindi{\textsf{Kind}_1}
\def\kindii{\textsf{Kind}_2}
\def\kindiii{\textsf{Kind}_3}

%\def\myitem{\vspace{.5cm}\item}

\def\derivable#1{\infer{#1}{\ldots}}
\def\parag{}


==> Macros/Macros_8PTSC.tex <==
\newcommand\SCons{{\mathcal S}}

\newcommand\RSTerms{{\mathcal Z}}
\newcommand\K{\mbox{$\Box$}}
\newcommand\T{\star}
\newcommand\Rel{{\mathcal R}}
\newcommand\Sort{{\mathcal A}}

\newcommand\xsubst{\textsf{xsubst}}

%Typing======================================
\newcommand\emptyenv{[]}
\newcommand\conv{\Rewsn{\B\x}}


\newcommand\DPTSC{\vdash_{\PTSC}}

\renewcommand\wf[1][\PTSC]{\hspace{5 pt}\textsf{wf}_{#1}}
%Previous def in Part1/Llxr_Macros



\newcommand\empt{\textsf{empty}}
\newcommand\extend{\textsf{extend}}
\newcommand\Ttyped{\textsf{sorted}}
\newcommand\Picons{\Pi\textsf{wf}}
\newcommand\Pir{\Pi\textsf{r}}
\newcommand\Pil{\Pi\textsf{l}}
\newcommand\convr{\textsf{conv}_r}
\newcommand\convl{\textsf{conv}_l}

\newcommand\subenv{\sqsubseteq}

%PTS==================================
\newcommand\DPTS{\vdash_{\PTS}}
\newcommand\DeriCoC[3]{{#1}\DPTS {#2}\col{#3}}


==> Macros/Macros_9DB.tex <==
%Sequent calculus of constructions

\newcommand\PTSCdb{\PTSC_{\sf{db}}}
\newcommand\PTSCi{\PTSC_{\sf{imp}}}

\newcommand\STermsdb{{\mathcal T}_{\sf{db}}}
\newcommand\SListsdb{{\mathcal L}_{\sf{db}}}

\newcommand\Pdb[3]{\Pi^{#2}{#3}}
\newcommand\lamidb[3]{\lambda^{#2}{#3}}
\newcommand\liftdb[3]{U^{#1}_{#2}{(#3)}}

\newcommand\cutjdb[4]{{#4}\{\hspace{-3pt}\{{{#3}\!\leftarrow\!{#2}}\}\hspace{-3pt}\}}
\newcommand\eln{{[\!]}}
\newcommand\appli[2]{#1(#2)}

\newcommand\compsup[1]{\overline{\sf{im}}(#1)}

\newcommand\cogg[2]{\pi^{#1}{(#2)}}
\newcommand\coggg[2]{\rho^{#1}{(#2)}}
\newcommand\ccdb[2]{{#2},{#1}}
\newcommand\DBname[2]{\overline{#2}^{\,#1}}
\newcommand\nameDB[2]{\underline{#2}_{\,#1}}
\newcommand\cofinG[1]{\phi_{#1}}



%Term reduction rules
\newcommand\Bdb{\textsf{B}_{\sf{db}}}
\newcommand\Aidb{\textsf{A1}_{\sf{db}}}
\newcommand\Aiidb{\textsf{A2}_{\sf{db}}}
\newcommand\Aiiidb{\textsf{A3}_{\sf{db}}}
\newcommand\Bidb{\textsf{B1}_{\sf{db}}}
\newcommand\Biidb{\textsf{B2}_{\sf{db}}}
\newcommand\Biiidb{\textsf{B3}_{\sf{db}}}
\newcommand\Bivdb{\textsf{B4}_{\sf{db}}}
\newcommand\Cidb{\textsf{C1}_{\sf{db}}}
\newcommand\Ciidb{\textsf{C2}_{\sf{db}}}
\newcommand\Ciiidb{\textsf{C3}_{\sf{db}}}
\newcommand\Ciiiidb{\textsf{C3'}_{\sf{db}}}
\newcommand\Civdb{\textsf{C4}_{\sf{db}}}
\newcommand\Cvdb{\textsf{C5}_{\sf{db}}}
\newcommand\Cvidb{\textsf{C6}_{\sf{db}}}
\newcommand\Cviidb{\textsf{C7}_{\sf{db}}}
\newcommand\Cviiidb{\textsf{C8}_{\sf{db}}}
\newcommand\Didb{\textsf{D1}_{\sf{db}}}
\newcommand\Diidb{\textsf{D2}_{\sf{db}}}
\newcommand\Diiidb{\textsf{D3}_{\sf{db}}}
\newcommand\Divdb{\textsf{D4}_{\sf{db}}}

\newcommand\Asdb{\textsf{As}_{\sf{db}}}
\newcommand\Bsdb{\textsf{Bs}_{\sf{db}}}
\newcommand\Csdb{\textsf{Cs}_{\sf{db}}}
\newcommand\Dsdb{\textsf{Ds}_{\sf{db}}}

\newcommand\xdb{\textsf{x}_{\sf{db}}}

\newcommand\Alldb{\Bdb\xdb}


%Typing

\newcommand\DeriTIdbf[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIdbsf[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTIdb[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriTIdbs[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTIdb{\hspace{5 pt}\textsf{wf}_{\sf{TS}_{\sf{db}}}}

\newcommand\TIdb{{\sf{TS}}_{\sf{db}}}
\newcommand\PSdb{{\sf{PS}}_{\sf{db}}}

\newcommand\DeriPSdb[3]{\Deri[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriPSdbs[4]{\Deris[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}


==> Macros/Macros_9Enumeration.tex <==
\ignore{
\newcommand\enum[5]{#2\sep #3\Longrightarrow #4\sep #5}
\newcommand\enums[6]{#2;#3\sep #4\Longrightarrow #5\sep #6}
}

\newcommand\enum[5]{\Deri{#2}{#4}{#3}\sep {#5}}
\newcommand\enums[6]{\Deris{#2}{#3}{#5}{#4}\sep {#6}}
\newcommand\goals[2]{#1\Longrightarrow #2}

\newcommand\PE{\textsf{PE}}

\newcommand\enumPS[5]{\Derip{\PE}{#2}{#4}{#3}\sep {#5}}
\newcommand\enumPSs[6]{\Derip{\PE}{#2;#3}{#5}{#4}\sep {#6}}
\newcommand\goalsPS[2]{#1\Longrightarrow_{\PE} #2}


\newcommand\constr[3]{#2\stackrel{#1}\longleftrightarrow #3}


==> Macros/Macros_9ProofSearch.tex <==
%Proof search


\newcommand\DPS{\vdash_{\textsf{PS}}}
\newcommand\PSS{\textsf{PS}}


\newcommand\DeriPS[3]{{#1}\DPS {#2}\col{#3}}
\newcommand\DeriPSs[4]{{#1};{#2}\DPS {#3}\col{#4}}

\newcommand\TtypedPS{\textsf{sorted}_\textsf{PS}}
\newcommand\contrs[1]{\textsf{sel.}_{#1}}
\newcommand\axPS{\textsf{ax}_\textsf{PS}}
\newcommand\PiconsPS{\Pi\textsf{wf}_\textsf{PS}}
\newcommand\PirPS{\Pi\textsf{r}_\textsf{PS}}
\newcommand\PilPS{\Pi\textsf{l}_\textsf{PS}}



==> Macros/Macros_9Tsynth.tex <==
%TI

\newcommand\Deric[3]{\Deri{#1}{#2}{\equiv\! #3}}
\newcommand\Derics[4]{\Deris{#1}{#2}{#3}{\equiv\! #4}}



\newcommand\DeriTIf[3]{\Deri[{\textsf{TS}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIsf[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTI[3]{\Deri[{\textsf{TS}}]{#1}{#2}{#3}}
\newcommand\DeriTIs[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTI{\hspace{5 pt}\textsf{wf}_{\textsf{TS}}}

\newcommand\extendTI{\textsf{extend}_\textsf{TS}}
\newcommand\axTI{\textsf{ax}_\textsf{TS}}
\newcommand\PiconsTI{\Pi\textsf{wf}_\textsf{TS}}
\newcommand\PirTI{\Pi\textsf{r}_\textsf{TS}}
\newcommand\PilTI{\Pi\textsf{l}_\textsf{TS}}

\newcommand\convp{\Rewsn{\B\x}}

\newcommand\expimp[1]{\Downarrow\!(#1)}
\newcommand\expimpname{\Downarrow}
\newcommand\TI{\textsf{TS}}
